Weak Stefan Formulation for Bulk Crystal Growth with Non-smooth Interfaces

Most heat transfer models for bulk crystal growth rely on the classical Stefan formulation to evaluate interface motion during phase change. However, when the interface is non-smooth the use of the classical Stefan formulation may lead to singularities. To address this problem, we propose a simulation model based on the weak formulation of the Stefan problem. Numerical solutions of the weak Stefan formulation are obtained using the finite volume method. This approach provides an energy conserving discretization scheme that accurately evaluates heat transfer around non-smooth interfaces. We apply the weak formulation to numerically simulate the solidification of silicon in the horizontal ribbon growth process. Results exhibit a limitation on the ribbon's pull speed, which previous classical Stefan models have failed to demonstrate. A comparison of heat transfer between radiation and gas cooling shows that gas cooling increases the pull speed limit for the same amount of heat removed.

==> sections/problem.tex <==
\section{Problem Statement}


 Figure 2 provides a cross-sectional schematic of the horizontal ribbon growth furnace around the growth tip of the ribbon. A cooling mechanism at the top surface of the melt (liquid) drives the solidification process which causes the single crystal ribbon (solid) to grow. Cooling takes place either through a passive mechanism, like radiation or through an active cooling system, like gas jets. The region around the growth tip, where the melt first solidifies and grows, is called the growth zone of the furnace. Preceding the growth zone is the replenishment zone that provides a constant supply of melt for the solidification process. The temperature of the melt in the replenishment zone is maintained by means of heaters placed inside the crucible walls of the furnace. The ribbon formed in the growth zone is extracted from the furnace by pulling it with a constant velocity, $v$. As the ribbon is being pulled, it passes through a stabilization zone that is set up to allow heat to conduct only in the vertical direction. This smoothens any irregularities on the bottom side of the ribbon and can also be used for thickness control. 
 
 We consider the process of solidification to take place inside a bounded domain $\Omega$, belonging to a subset of the Euclidean space $\mathbf{R}^n$ $(n=2,3)$. We shall assume that the process occurs at a constant volume i.e., no volume change associated with phase change. The domain is occupied by a pure material capable of attaining two phases, liquid and solid, at a sharp melting point $T_m$. To simplify fluid motion, the material is assumed to move at a uniform speed, $v$, throughout the domain. The analysis is carried out in a Lagrangian frame of reference, so the material appears stationary in this reference frame. 
 
 The time interval for analysis is set to $]0,\tau [$, where $\tau$ is a constant. We define $Q:=\Omega\times]0,\tau [$, and $Q_s$ and $Q_l$ the subset of Q that correspond to the solid and liquid phases respectively. The energy balance in each phase can be written in the strong form as:
 \begin{equation} \label{eq:classical_stefan1}
     \frac{\partial \rho c_i T}{\partial t}-k_i\nabla^2T=0\qquad\text{in }Q_i,\quad i=s,l
 \end{equation}
 where $\rho$ is density, $c$ is the heat capacity, $k$ is the thermal conductivity and $T$ is the absolute temperature field of the material. The subscripts $s$ and $l$ are used to denote solid and liquid phases respectively.
 
 The solid and liquid phases are separated by a space-time manifold, $I:=\partial Q_s\cap\partial Q_l$, in $\mathbf{R}^{n+1}$ that represents the collection of solid-liquid interfaces. At any instant $t\in[0,\tau]$, let the instantaneous interface be defined by a smooth surface $I_t:=I\cap(\Omega\times{t})$. The interface will evolve continuously based on the conservation law:
 \begin{equation}\label{eq:classical_stefan2}
    \Big[k_l\nabla T_l-k_s\nabla T_s\Big].\,\hat{n}=-\rho L \,\Vec{v}.\hat{n}  \qquad\text{on   }I,
 \end{equation}
 where $\hat{n}\in\mathbf{R}^n$ is a unit vector field normal to $I_t$ oriented from the solid to the liquid phase. $\nabla T_i$ denotes the gradient of the temperature field on $I$ relative to the $i$ phase. $L$ is the latent heat of fusion, $\Vec{v}.\hat{n}$ denotes the normal velocity of the interface from solid to liquid. Equations \eqref{eq:classical_stefan1} and \eqref{eq:classical_stefan2} together are known as the strong form or the classical formulation of the Stefan problem. 
\begin{figure}[ht]
\centering
  \centering
  \includegraphics[width=1\linewidth]{figs/problem.pdf}
  \caption{The Sharp edge at the growth tip position makes it unfitting to use the classical Stefan formulation}
  \label{fig:motivation}
\end{figure}

A major assumption in the classical formulation of the Stefan problem is that the solid-liquid interface $I_t$ is smooth for all $t\in[0,\tau]$ and the unit normal is defined everywhere on the interface. This is a very restrictive assumption given that we routinely come across non-smooth interfaces in crystal growth. Figure~\ref{fig:motivation} provides two example of frequently encountered situation in crystal growth where the classical Stefan formulation is not applicable. Figure~\ref{fig:motivation}a is a close-up of a crystal growth configuration around the triple point. The solidification interface makes an angle $\theta$ with the free surface. In the case of a faceted growth, as observed in \cite{kellerman2013floating,helenbrook2016experimental, kellerman2016floating}, $\theta$ can be a fixed angle to the free surface. As we can see, the unit normal is uniquely defined everywhere on the interface except at the triple point. At the triple point, the tip grows with a velocity of either $v$ or $v \sin\theta$ depending on the observers viewing from $\hat{n}_1$ or $\hat{n}_2$, respectively. This presents an ambiguity in the choice of the normal velocity to be used in eq.~\eqref{eq:classical_stefan2} at the tip. A similar problem occurs in systems with facet growth, as shown in figure~\ref{fig:motivation}b, where the normal component of the interfacial velocity cannot be defined~\cite{fujiwara2012crystal,lau2020situ,hu2020situ}.

Incorrect knowledge on the evolution of the interface may lead to erroneous predictions of crystal geometry which may cause problems in the calculation of energy, mass and momentum transport (Brandon, 2003). Using the classical Stefan formulation to model interfaces that are non-smooth can lead to incorrect results~\cite{segal1998conserving,vuik2000conserving,king1999two}. This is because the limit of the energy balance equation on an arbitrarily small neighbourhood of a non-differentiable interface does not exist and only the integral form of the energy balance makes sense. In the context of the horizontal ribbon growth process, this has made an accurate analysis of the heat transfer at the growth tip impossible. The impact of this discrepancy in models of other crystal growth processes has not been determined (ramachandran, 2009).







